On Rendering Synthetic Images for Training an Object Detector

We propose a novel approach to synthesizing images that are effective for training object detectors. Starting from a small set of real images, our algorithm estimates the rendering parameters required to synthesize similar images given a coarse 3D model of the target object. These parameters can then be reused to generate an unlimited number of training images of the object of interest in arbitrary 3D poses, which can then be used to increase classification performances. A key insight of our approach is that the synthetically generated images should be similar to real images, not in terms of image quality, but rather in terms of features used during the detector training. We show in the context of drone, plane, and car detection that using such synthetically generated images yields significantly better performances than simply perturbing real images or even synthesizing images in such way that they look very realistic, as is often done when only limited amounts of training data are available.

==> Makefile <==
# Enter here the name of the document (without .tex extension)
doc = top

PDFLATEX = pdflatex --shell-escape
# type "make" to process latex
# type "make refs" to get proper references to figures and papers
# "make ps" and "make pdf" do what you imagine
# "make clean" removes the *~ files of emacs
# "make hardclean" removes the .dvi .aux .log .blg files and the postscript document

quick: 
	@$(PDFLATEX) $(doc).tex || latex $(doc).tex
	@cat $(doc).log | grep "LaTeX Warning:" || echo "No warning."
	@cat $(doc).log | grep "Output written"

ns: 
	@pdflatex -interaction=batchmode $(doc).tex || cat $(doc).log | grep "LaTeX Error:"
#	@cat $(doc).log | grep "LaTeX Warning:" || echo "No warning."
	@cat $(doc).log | grep "Output written"

refs: 
	@pdflatex -interaction=batchmode $(doc).tex || latex $(doc).tex
	@bibtex $(doc)
	@pdflatex -interaction=batchmode $(doc).tex
	@pdflatex -interaction=batchmode $(doc).tex
	@cat $(doc).log | grep "LaTeX Warning:" || echo "No warning."
	@cat $(doc).log | grep "Output written"

up:
	cvs update

co:	commit
commit:
	cvs commit

ps:     refs
	dvips -o $(doc).ps -t letter $(doc).dvi

pdf:	
	latex -interaction=batchmode $(doc).tex || latex $(doc).tex
	bibtex $(doc)
	latex $(doc).tex
	latex $(doc).tex
	dvips -o $(doc).ps -t letter $(doc).dvi
	ps2pdf $(doc).ps
	acroread $(doc).pdf

clean:
	\rm -f *~ 

hardclean:
	\rm -f $(doc).dvi $(doc).ps $(doc).pdf *~ *.aux *.log *.blg *.bbl


==> Makefile_cvpr <==
# Enter here the name of the document (without .tex extension)
doc = top

PDFLATEX = pdflatex
# type "make" to process latex
# type "make refs" to get proper references to figures and papers
# "make ps" and "make pdf" do what you imagine
# "make clean" removes the *~ files of emacs
# "make hardclean" removes the .dvi .aux .log .blg files and the postscript document

quick: 
	@$(PDFLATEX) $(doc).tex || latex $(doc).tex
	@cat $(doc).log | grep "LaTeX Warning:" || echo "No warning."
	@cat $(doc).log | grep "Output written"

ns: 
	@pdflatex -interaction=batchmode $(doc).tex || cat $(doc).log | grep "LaTeX Error:"
#	@cat $(doc).log | grep "LaTeX Warning:" || echo "No warning."
	@cat $(doc).log | grep "Output written"

refs: 
	@pdflatex -interaction=batchmode $(doc).tex || latex $(doc).tex
	@bibtex $(doc)
	@pdflatex -interaction=batchmode $(doc).tex
	@pdflatex -interaction=batchmode $(doc).tex
	@cat $(doc).log | grep "LaTeX Warning:" || echo "No warning."
	@cat $(doc).log | grep "Output written"

up:
	cvs update

co:	commit
commit:
	cvs commit

ps:     refs
	dvips -o $(doc).ps -t letter $(doc).dvi

pdf:	
	latex -interaction=batchmode $(doc).tex || latex $(doc).tex
	bibtex $(doc)
	latex $(doc).tex
	latex $(doc).tex
	dvips -o $(doc).ps -t letter $(doc).dvi
	ps2pdf $(doc).ps
	acroread $(doc).pdf

clean:
	\rm -f *~ 

hardclean:
	\rm -f $(doc).dvi $(doc).ps $(doc).pdf *~ *.aux *.log *.blg *.bbl


==> abstract.tex <==
%% -*- mode: latex; mode: reftex; mode: flyspell; TeX-master: "top.tex"; -*-

\begin{abstract}

We  propose a  novel  approach to  synthesizing images  that  are effective  for
training  object detectors.   Starting  from a  small set  of  real images,  our
algorithm  estimates the  rendering  parameters required  to synthesize  similar
images given a coarse  3D model of the target object.  These parameters can then
be reused to  generate an unlimited number  of training images of  the object of
interest  in   arbitrary  3D  poses,  which   can  then  be  used   to  increase
classification performances.

A key insight of our approach  is that the synthetically generated images should
be similar to real images, not in terms of image quality, but rather in terms of
features used during the classifier training.  We show in the context of
  drone, plane, and car detection that using such synthetically generated images
  yields significantly better performances than simply perturbing real images or
  even synthesizing  images in  such a way  that they look  very realistic,  as is
  often done when only limited amounts of training data are available.

% \keywords{synthetic image generation, object detection}

\end{abstract}


==> cover.tex <==
% Example of title page for the projects carried out within the lasec

% Simply include it in your mastex tex file:
%        \input{cover}


% Updated March 2006 (SP)


\newcommand{\logoepfl}[0]{
  \begin{center}
    \includegraphics[width=4cm]{./fig/logo_epfl_coul.pdf}
  \end{center}
  \vspace{0.3cm}
  \hrule
}
%\newcommand{\logolasec}[0]{
%  \vspace{1cm}
%  \hrule
%  \begin{center}
%    \includegraphics[width=4.5cm]{logo_lasec_coul.eps}
%  \end{center}
%}
\newcommand{\project}[1]{
  \vspace{1cm}
  \begin{center}
    \begin{normalsize}{
        \bf #1}
    \end{normalsize}
  \end{center}
}
\newcommand{\department}[1]{ 
 \vspace{0.9cm}
  \begin{center}
    \large{#1}
  \end{center}
  \vspace{0.9cm}
}
\newcommand{\supervisor}[1]{
  \begin{center}
    \begin{normalsize}{
        \bf #1}
    \end{normalsize}
  \end{center}
}
\renewcommand{\author}[1]{
  \begin{center}
    \large{#1}
  \end{center}
}
\renewcommand{\title}[1]{
  \vspace{1cm}
  \begin{center}
    \huge{#1}
  \end{center}
  \vspace{0.7cm}
}
\renewcommand{\date}[2]{
  \begin{center}
    \normalsize{ #1 #2}
  \end{center}
  \vspace{0.5cm}
}


\thispagestyle{empty}


% begin title page
  \logoepfl

%  \project{Semester Project}

%  \department{CVLAB}

%  \date{January}{2013}
  
  \renewcommand{\thefootnote}{\ifcase\value{footnote}\or*\or($\nfty$)\fi}
  
  \title{On Rendering Synthetic Images for Training an Object Detector}

  \author{Artem Rozantsev (artem.rozantsev@epfl.ch)}
  \author{Vincent Lepetit (vincent.lepetit@epfl.ch)}
  \author{Pascal Fua (pascal.fua@epfl.ch)}

\department{School of Computer and Communication Sciences Swiss Federal Institute of Technology, Lausanne (EPFL)}

\vspace{4cm}

\project{Technical Report}
\date{June 16, 2014}



% end title page


